Deep Reinforcement Learning for Cyber System Defense under Dynamic Adversarial Uncertainties

Development of autonomous cyber system defense strategies and action recommendations in the real-world is challenging, and includes characterizing system state uncertainties and attack-defense dynamics. We propose a data-driven deep reinforcement learning (DRL) framework to learn proactive, context-aware, defense countermeasures that dynamically adapt to evolving adversarial behaviors while minimizing loss of cyber system operations. A dynamic defense optimization problem is formulated with multiple protective postures against different types of adversaries with varying levels of skill and persistence. A custom simulation environment was developed and experiments were devised to systematically evaluate the performance of four model-free DRL algorithms against realistic, multi-stage attack sequences. Our results suggest the efficacy of DRL algorithms for proactive cyber defense under multi-stage attack profiles and system uncertainties.

==> AAAI_2023_RL_Cyberv2 (1)/figures/tiered_rl.tex <==
\section{Constrained Reinforcement Learning}
A key aspect of AI assurance in cyber systems is safety, guaranteeing that a defense strategy computed by an AI agent does not violate system stability requirements. In this flash talk, we will briefly discuss an online approach to train an AI agent tasked with optimizing cyber defense decisions. Our tiered approach includes transforming coarse-grained defense strategies computed by reinforcement learning into fine-grained safe-by-construction defense actions through formal verification via satisfiability modulo theories.

{\color{red}} Pick the model which one is best --- which is DQN

==> figures/tiered_rl.tex <==
\section{Constrained Reinforcement Learning}
A key aspect of AI assurance in cyber systems is safety, guaranteeing that a defense strategy computed by an AI agent does not violate system stability requirements. In this flash talk, we will briefly discuss an online approach to train an AI agent tasked with optimizing cyber defense decisions. Our tiered approach includes transforming coarse-grained defense strategies computed by reinforcement learning into fine-grained safe-by-construction defense actions through formal verification via satisfiability modulo theories.

{\color{red}} Pick the model which one is best --- which is DQN
